Exploiting flux ratio anomalies to probe warm dark matter in future large scale surveys

Flux ratio anomalies in strong gravitationally lensed quasars constitute a unique way to probe the abundance of non-luminous dark matter haloes, and hence the nature of dark matter. In this paper we identify double imaged quasars as a statistically efficient probe of dark matter, since they are 20 times more abundant than quadruply imaged quasars. Using N-body simulations that include realistic baryonic feedback, we measure the full distribution of flux ratios in doubly imaged quasars for cold (CDM) and warm dark matter (WDM) cosmologies. Through this method, we fold in two key systematics - quasar variability and line-of-sight structures. We find that WDM cosmologies predict a ~6 per cent difference in the cumulative distribution functions of flux ratios relative to CDM, with CDM predicting many more small ratios. Finally, we estimate that ~600 doubly imaged quasars will need to be observed in order to be able to unambiguously discern between CDM and the two WDM models studied here. Such sample sizes will be easily within reach of future large scale surveys such as Euclid. In preparation for this survey data we require discerning the scale of the uncertainties in modelling lens galaxies and their substructure in simulations, plus a strong understanding of the selection function of observed lensed quasars.

==> table-1.tex <==
\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
Sample & $\epsilon$ (kpc / h ) &$\sigma_{DM}/m$ (cm$^2$/g) &$N_{\rm cl}$ & $N_{\rm eff}$ &\textcolor{red}{$\langle \log_{10} M_{\rm tot}/M_{\odot}\rangle$ or $\log_{10} \langle M_{\rm tot}/M_{\odot}\rangle$} \\
\hline
CDM & 4 & 0.0 & 1366 &  466 & 14.45 \\ 
SIDM0.1 & 4 & 0.1 & 1344 &  731 & 14.32 \\ 
SIDM0.3 & 4 & 0.3 & 1374 &  672 & 14.42 \\ 
SIDM & 4 & 1.0 & 1330 &  644 & 14.40 \\ 
CDM-hires & 2 & 0.0 &   80 &   13 & 14.23 \\ 
SIDM-hires & 2 & 1.0 &   95 &   18 & 14.25 \\ 
obs & 0 & 0.0 &   10 &   10 & 15.08 \\ 
\hline
\end{tabular}
\caption{ The sample selection of galaxy clusters from the simulations with their corresponding dark matter cross-section. The third column gives the total number of clusters extracted from the simulation and the fourth column gives the number of relaxed clusters after cuts. The final column gives the mean halo mass of the cut sample.
\label{tab:data}}
\end{table*}

